Exponential Lower Bounds for Locally Decodable and Correctable Codes for Insertions and Deletions

Locally Decodable Codes (LDCs) are error-correcting codes for which individual message symbols can be quickly recovered despite errors in the codeword. LDCs for Hamming errors have been studied extensively in the past few decades, where a major goal is to understand the amount of redundancy that is necessary and sufficient to decode from large amounts of error, with small query complexity. In this work, we study LDCs for insertion and deletion errors, called Insdel LDCs. Their study was initiated by Ostrovsky and Paskin-Cherniavsky (Information Theoretic Security, 2015), who gave a reduction from Hamming LDCs to Insdel LDCs with a small blowup in the code parameters. On the other hand, the only known lower bounds for Insdel LDCs come from those for Hamming LDCs, thus there is no separation between them. Here we prove new, strong lower bounds for the existence of Insdel LDCs. In particular, we show that $2$-query linear Insdel LDCs do not exist, and give an exponential lower bound for the length of all $q$-query Insdel LDCs with constant $q$. For $q \ge 3$ our bounds are exponential in the existing lower bounds for Hamming LDCs. Furthermore, our exponential lower bounds continue to hold for adaptive decoders, and even in private-key settings where the encoder and decoder share secret randomness. This exhibits a strict separation between Hamming LDCs and Insdel LDCs. Our strong lower bounds also hold for the related notion of Insdel LCCs (except in the private-key setting), due to an analogue to the Insdel notions of a reduction from Hamming LCCs to LDCs. Our techniques are based on a delicate design and analysis of hard distributions of insertion and deletion errors, which depart significantly from typical techniques used in analyzing Hamming LDCs.

==> 2q-nonlinear.tex <==
\section{Conjectures about 2-query non-linear LDCs}

In this section we investigate the possibility of 2-query non-linear LDCs. We will view individual bits of the codeword as $\mathbb{F}_2$-polynomials (of degree at most $n$), i.e. $C_i(\*x) = \sum_{S\subseteq [n]}a_{i, S} \*x^S$ where $\*x^S \coloneqq \prod_{j \in S}x_j$ and $a_{i,S} \in \mathbb{F}_2$.

As the first step we focus on codes which are good on average. Specifically, we want to design a code $C \colon \mathbb{F}_2^n \rightarrow \mathbb{F}_2^m$ with the following property.

\paragraph{Candidate Property} There exists $c > 1$ such that for any $k \in [n]$, there is $\sigma_k \in \mathbb{F}_2$ satisfying
\begin{align*}
	\E_{(i,j) \in P_k}\left[ \Pr_{\*x \in \mathbb{F}_2^n}\left[ C_i(\*x) + C_j(\*x) + x_k + \sigma_k = 0 \right] \right] > \frac{1}{2} + \eps.
\end{align*}
Here $P_k \subseteq \binom{[m]}{2}$ contains all pairs $(i,j)$ satisfying $c^{k-1} \le \abs{i-j} < c^k$.

\begin{conjecture}
Candidate Property implies $2$-query insdel LDCs which are good on average.
\end{conjecture}

\jeremiah{Idea: Given a ins/deletion pattern call an index $t$ of the codeword is $\alpha$-good if for every $t$ the fraction of insertions/deletions in the range $[t,t+r]$ and $[t-r,t]$ is at most $\alpha$. We can argue that most indices must $\alpha$-good as long as the total number of ins/del errors is bounded. If an index $t$ is $\alpha$-good and we query for a random pair $(i,j) \in P_k \cap [t-r,t+r]^2$ then we should be able to argue that the decoder has a good chance of succeeding  }

\jeremiah{Note: A good on average 2-query insdel LDC should yield a (weaker version of a) 2-query private key insdel LDC by XORing the input message with a one-time pad to get a random message. Note: May need to relax definition of private key insdel LDC to say that for any particular index $i$ the decoder succeeds with advantage $\epsilon$ with the randomness taken over the coins of the channel/decoder and the selection of the private key. The stronger version of private key insdel LDCs says that the channel fails to ``fool" the decoder i.e., {\em after} the channel outputs the corruption the decoder we can say that for all $i$ the decoder succeeds with probability $\epsilon$ }

\subsection{Quadratic polynomials}
Let $p(\*x) = \*x^\top Q \*x + \*a^\top \*x + b$ be a quadratic polynomial, where $Q \in \mathbb{F}_2^{n \times n}$ is an upper-triangular matrix. We can absorb the diagonal elements of $Q$ into the linear term $\*a^\top \*x$ and assume $Q$ has zeros on the diagonal. We will show that the number of zeros of $p$ depends only on the rank of $Q$ (and we will also call it the rank of $p$).
 
Suppose $Q$ has rank $2h$ for some integer $h \le n/2$. Dickson's Theorem (\cite{macwilliams1977theory} Chapter 15, Theorem 4) says that there exists an invertible $R \in \mathbb{F}_2^{n \times n}$ such that for $\*y = R\*x$, we have
\begin{align*}
\*y^\top Q \*y = \*x^\top (R^\top Q R) \*x = \sum_{j=1}^{h}x_{2j-1}x_{2j}.
\end{align*}
Therefore for $\*a' = \*a^\top R$ and some $\sigma = \sigma(p) \in \mathbb{F}_2$ we can write 
\begin{align*}
	p(\*y) = \sum_{j=1}^{h}\tp{ x_{2j-1}x_{2j} + a_{2j-1}'x_{2j-1} + a_{2j}'x_{2j} } + b = \sum_{j=1}^{h}\tp{x_{2j-1} + a_{2j}'} \tp{x_{2j} + a_{2j-1}'} + \sigma.
\end{align*}
\xnote{Is there something wrong here? I think the part of $\*a^\top R x$ can have other $x_i$'s besides those with index in $[2h]$?}

\minshen{I agree that there should be some additional linear terms which may alter the number of zeros. We may want to look deeper into the weight distribution of 2nd-order Reed-Muller codes then.}

Since $R$ is invertible we only need to understand the number of zeros of the polynomial $f(\*x) = \sum_{j=1}^{h}x_{2j-1}x_{2j}$, which is given by the following proposition.

\begin{proposition}
The polynomial $f(\*x) = \sum_{j=1}^{h}x_{2j-1}x_{2j}$ has $2^{2h-1} + 2^{h-1}$ zeros.
\end{proposition}

In particular, if the rank of $p$ is $2h \le n-1$ and $\sigma(p) = 0$, we have that
\begin{align*}
	\Pr_{\*x \in \mathbb{F}_2^n}\left[ p(\*x) = 0 \right] = \frac{2^{n-2} + 2^{(n-3)/2}}{2^n} = \frac{1}{4} + 2^{-(n+3)/2}.
\end{align*}
Similarly, if $\sigma(p) = 1$ then the probability is $3/4 - 2^{-(n+3)/2}$.

The following conjecture implies codes with Candidate Property.

\begin{conjecture}
There are quadratic polynomials $C_1, \dots, C_m$ and $c > 1$, such that for every $k \in [n]$ and most $(i,j) \in [m] \times [c^{k-1}, c^k)$ the polynomial $p_{i,j,k}(\*x) = C_i(\*x) + C_j(\*x) + x_k$ has rank at most $n-1$. Moreover, these polynomials have the same $\sigma$.
\end{conjecture}



\section{Hypercontractivity Theorem for Matrix-valued Functions}

\begin{definition}[Schatten $p$-norm]
Let $p \in [1,+\infty)$. For matrix $M$ with singular values $\sigma_1,\dots, \sigma_d$, define its Schatten $p$-norm to be $\norm{M}_p \coloneqq \tp{\frac{1}{d}\sum_{i=1}^{d}\sigma_i^p}^{1/p}$.
\end{definition}

Below are some properties of $\norm{\cdot}_p$.
\begin{proposition}
Let $p, q \in [1,+\infty)$ be such that $1/p + 1/q=1$.
\begin{itemize}
    \item (Unitarily invariant) If $U$, $V$ are unitary matrices, we have $\norm{M}_p = \norm{UMV^{\dag}}_p$.
    \item (Duality) $\norm{S}_p = \sup\set{\langle S, T \rangle \colon \norm{T}_q=1}$ where $\langle S, T \rangle \coloneqq \Tr(S^{\dag}T)$.
    \item (Non-increasing under pinchings) Let $P_1, \dots, P_k$ be a set of mutually orthogonal projection matrices such that $P_1 + \dots + P_k = I$. Then we have
    \begin{align*}
        \norm{M}_p \ge \norm{P_1MP_1 + \dots + P_k MP_k}_p.
    \end{align*}
\end{itemize}
\end{proposition}

The following theorem is proven in~\cite{Ben-AroyaRW08}.
\begin{theorem}
Let $f \colon \set{\pm 1}^n \rightarrow \mathbb{R}^{m \times m}$ be a matrix-valued Boolean function. For $1\le p\le 2$ we have
\begin{align*}
    \tp{\sum_{S\subseteq [n]}(p-1)^{|S|}\norm{\widehat{f}(S)}_p^2}^{1/2} \le \tp{\frac{1}{2^n}\sum_{x \in \set{\pm 1}^n}\norm{f(x)}_p^p}^{1/p}.
\end{align*}
\end{theorem}

==> Hadamard.tex <==
\section{Hadamard Code is Not a 2-query Insdel LDC}
We consider the Hadamard Code under any arbitrary permutation. Let $n$ be the message length and $N=2^n$ be the codeword length. We assume the decoder has the following form:

For a message $x \in \{0, 1\}^n$, to decode $x_i$, the decoder uses a fixed partition of $[N]$ into $N/2$ disjoint pairs $Q^i=\{(s^i_r, t^i_r)\}$ for $r \in [N/2]$. The decoder samples a pair from $Q^i$ using an arbitrary fixed distribution (the uniform distribution as in the standard decoder is a special case), and outputs $y_{s^i_r} \oplus y_{t^i_r}$, where $y$ is the encoding of $x$. Note that for different $i, j \in [n]$, we have $Q^i \cap Q^j =\emptyset$.

WLOG assume that $\forall r, s^i_r \leq t^i_r$, and let $\ell^i_r=t^i_r-s^i_r \geq 0$ be the distance between the two indices. For any $i$, define the set $L^i=\{r \in [N/2]: \ell^i_r \geq n^{2/3}\}$.

We first have the following claim.

\begin{claim}
There exists $i \in [n]$ s.t. $|L^i| \geq (1-\frac{4}{n^{1/3}})\frac{N}{2}$.
\end{claim}

\begin{proof}
There are at most $N(\lfloor n^{2/3} \rfloor+1) \leq 2 N n^{2/3}$ pairs of ordered indices $(s, t)$ s.t. $|s-t| < n^{2/3}$. Thus there exists $i \in [n]$ s.t. the number of such pairs in $Q^i$ is at most $2 N/(n^{1/3})$ and the claim follows.
\end{proof}

From now on we fix such an $i$, and for convenience we drop the superscript $i$ and just use $(s_r, t_r)$ to stand for $(s^i_r, t^i_r)$. Fix any constant $\alpha \in (0, 1/6)$, we consider the following edit operations on the codeword $y$: for each bit of $y$, independently delete it with probability $\alpha$. After this we insert some number of bits at the end to make sure the new string $\tilde{y}$ still has length $N$.

Now consider any pair of indices $(s_r, t_r) \in Q^i$ and the corresponding bits $(\tilde{y}_{s_r}, \tilde{y}_{t_r})$ after the operations. We have two cases:

\begin{enumerate}
    \item At least one corresponding bit is an inserted bit, in which case we say $(s_r, t_r)$ is \emph{bad} for this sequence of edit operations.
    \item Both bits are bits in the original codeword. In this case $(s_r, t_r)$ corresponds to some pair of indices $(s'_r, t'_r)$ in the original codeword. Note that by our operations, we always have $s'_r \geq s_r$ and $t'_r \geq t_r$ since $s_r=s'_r-\text{number of deletions before the index } s'_r$, and the same for $t_r$. In addition, $t'_r-s'_r \geq t_r-s_r$. Now, if $(s'_r, t'_r) \in Q^i$ we say the pair $(s_r, t_r)$ is \emph{good} for this sequence of edit operations, otherwise we say $(s_r, t_r)$ is \emph{bad} for this sequence of edit operations
\end{enumerate}

Our key idea is to bound the probability that a pair $(s_r, t_r) \in L^i$ is good, and we do this as follows.

First, if $\tilde{y}_{s_r}$ is an inserted bit then clearly $(s_r, t_r)$ is bad. Now assume this is not the case and $\tilde{y}_{s_r}$ corresponds to some index $s'_r$ in the original codeword. We can first fix $s'_r$ and the deletions up to index $s'_r$, so that $s_r$ corresponds to $s'_r$. Observe that there is at most one pair in $Q^i$ where the left index is equal to $s'_r$ (it's possible that no such pair exists, in which case $(s_r, t_r)$ is also bad). Assume that there is indeed such a pair $(s'_r, t'_r) \in Q^i$. Now if $t'_r -s'_r < t_r-s_r$ then again it is impossible for $(s_r, t_r)$ to correspond to $(s'_r, t'_r)$ and hence $(s_r, t_r)$ is bad.

Finally, if $t'_r -s'_r \geq t_r-s_r$, then as $(s_r, t_r) \in L^i$ we have $t_r-s_r \geq n^{2/3}$ and thus also $t'_r -s'_r \geq n^{2/3}$. Conditioned on all the deletions we have fixed, the remaining deletions still happen independently with probability $\alpha$. In order for $(s_r, t_r)$ to correspond to $(s'_r, t'_r)$, we need the number of deletions that happen between $s'_r$ and $t'_r$ to be exactly equal to $(t'_r -s'_r)-(t_r-s_r)$. However note that the number of deletions in this range is a binomial distribution with parameter $\alpha$, and thus we can use anti-concentration. Specifically, the maximum probability mass of any support in this binomial distribution is $\frac{\beta}{\sqrt{t'_r -s'_r}} \leq \frac{\beta}{n^{1/3}}$ where $\beta$ is a constant depending on $\alpha$. To conclude, we have the following claim.

\begin{claim}
For any pair $(s_r, t_r) \in L^i$, \[\Pr[(s_r, t_r) \text{ is good}] \leq \frac{\beta}{n^{1/3}},\] where the probability is over the sequence of random deletions.
\end{claim}

Now suppose the decoder puts probability mass $p$ on the pairs in $L^i$, and probability mass $q$ on the pairs in $Q^i \setminus L^i$, with $p+q=1$. Then by linearity of expectation we have

\[E[\text{decoder's probability mass on good pairs in } L^i] \leq \frac{\beta p}{n^{1/3}},\]
where the expectation is over the sequence of random deletions. Now by Markov's inequality 

\[\Pr[\text{decoder's probability mass on good pairs in } L^i \geq \frac{2\beta p}{n^{1/3}}] \leq 1/2.\]

By Chernoff bound, with probability $1-2^{-\Omega(N)}$ the number of deletions (and hence also the number of insertions) is at most $2\alpha N$. Therefore, there exists a sequence of at most $4 \alpha N$ insertions and deletions, s.t. the decoder's probability mass on good pairs in $L^i$ is at most $\frac{2\beta p}{n^{1/3}}$.

Next, based on the above sequence of operations, we can use substitutions to destroy all pairs in $Q^i \setminus L^i$. Since we have at most $2 N/(n^{1/3})$ such pairs, no matter what these pairs become after the insertions and deletions, we can use at most $2 N/(n^{1/3})=o(N)$ substitutions to destroy them, and these pairs also become bad. So finally we have the decoder's probability mass on good pairs is at most $\frac{2\beta p}{n^{1/3}}$, with a sequence of at most $5 \alpha N$ edit operations.

Now fix the bit $x_i$ we want to decode, and choose uniformly random bits for the insertions, substitutions and the other bits in $x$. Then for any bad pair, the output of the decoder is going to be completely independent of $x_i$. Therefore, there exists a choice such that the decoder's success probability on the bad pairs is at most half the probability mass of the bad pairs. Hence, the total success probability of the decoder in this case is  at most $1/2+\frac{\beta p}{n^{1/3}}=1/2+o(1)$.

==> questions.tex <==


\section{Some Questions}
\begin{enumerate}
	\item Can we construct a 2-query InsDel LDC? For any arbitrary rate?
	
	\item It seems an adaptive decoder is needed for an InsDel LDC.
	Is this the case? Could we construct a non-adaptive InsDel LDC?
	
	\item Is the long code a good InsDel LDC? \url{https://en.wikipedia.org/wiki/Long_code_(mathematics)}
	
	\item What techniques beyond using smooth codes can we use to get lower bounds?
	
	\item For Hamming codes, a smooth code can be converted into a Hamming code.
	This seems impossible for InsDel.
	Is this the case?
\end{enumerate}

==> rLDC-lb.tex <==
\section{Lower bounds for relaxed insdel LDCs}

The following definition is adapted from Definition 3.2 of~\cite{gur2019lower}.

\begin{definition}[Strong rILDC]
A code $C \colon \Sigma^n \rightarrow \Sigma^m$ is a $(q,\delta,\alpha,\rho)$-relaxed insdel LDC (rILDC) if there exists a probabilistic algorithm $\Dec$ with the following properties.
\begin{itemize}
\item \textsf{(Perfect) Completeness:} For every $x \in \Sigma^n$ and $i \in [n]$, it holds that 
\begin{align*}
\Pr[\Dec(C(x), m, i) = x_i] = 1.
\end{align*}
\item \textsf{Relaxed Decoding:} For every $x \in \Sigma^n$ and $y \in \Sigma^{m'}$ such that $\ED\tp{C(x), y} \le \delta \cdot 2m$, and for every $i \in [n]$, we have
\begin{align*}
	\Pr\left[ \Dec(y, m', i) \in \set{x_i, \perp} \right] \ge \alpha.
\end{align*}
\item \textsf{Success Rate:} For every $x \in \Sigma^n$ and $y \in \Sigma^{m'}$ such that $\ED\tp{C(x), y} \le \delta \cdot 2m$, there exists a set $I_y \subseteq [n]$ of size $\abs{I_y} \ge \rho n$ such that for every $i \in I_y$, we have
\begin{align*}
	\Pr\left[ \Dec(y, m', i) = x_i \right] \ge \alpha.
\end{align*}
\end{itemize}
Furthermore, in every invocation, $\Dec$ reads at most $q$ symbols of $y$. The probabilities are taken over the randomness of $\Dec$, and $\ED\tp{C(x),y}$ denotes the minimum number of insertions/deletions necessary to transform $C(x)$ into $y$.
\end{definition}

\textcolor{red}{Can we prove the following lemma?}

\begin{lemma}
Let $C \colon \set{0,1}^n \rightarrow \set{0,1}^m$ be a $(q,\delta,\alpha,\rho)$-relaxed insdel LDC. Suppose $\rho\alpha + (1-\rho)\alpha/2 = 1/2+\eps$ for some $\eps > 0$. Then there exists a decoder $\Dec$ and a subset $I \subseteq [n]$ of size at least $\eps n$ such that for every $i \in I$, we have 
\begin{align*}
	\Pr_{i \in [n]}\left[ \Dec(y, m', i) = x_i \right] \ge \frac{1}{2} + \frac{\eps}{2}.
\end{align*}
The probability is taken over the uniform random choice of $x \in \set{0,1}^n$, and the random string $y$ which is obtained by applying the deletion process to $C(x)$, and the randomness of $\Dec$.
\end{lemma}
\begin{proof}[Proof Sketch]
Let $\Dec_0$ be the relaxed decoder for $C$. The local decoder $\Dec$ will simulate $\Dec_0$ and output the result, except when $\Dec_0$ returns ``$\perp$'', $\Dec$ instead returns a uniform random bit. 

We note that our error distribution introduces at most $\delta \cdot 2m$ insdel errors with high probability ($\ge 1-\negl(n)$). Therefore by definition of relaxed LDCs, for a random index $i \in [n]$, we have (roughly)
\begin{align*}
    \Pr\left[ \Dec(y, m', i) = x_i \right] \ge \rho\alpha + \tp{1 - \rho} \cdot \frac{\alpha}{2}= \frac{1}{2} + \eps.
\end{align*}
By a Markov-type argument, there is a subset $I \subseteq [n]$ of size at least $\eps n$ such that for all $i \in [n]$, we have
\begin{align*}
    \Pr\left[ \Dec(y,m',i)=x_i \right] \ge \frac{1}{2} + \frac{\eps}{2}.
\end{align*}
\end{proof}


\textcolor{red}{
Open problems:
\begin{itemize}
\item For insdel errors, do first two conditions implies the third?
\item What about the case $\rho\alpha \le 1/2$ for relaxed insdel LDCs? Constructions/Lower bounds?
\item Relaxed insdel LCCs?
\item Implications of insdel LDCs/LCCs?
\end{itemize}
}
